Robustness of Explanation Methods for NLP Models

Explanation methods have emerged as an important tool to highlight the features responsible for the predictions of neural networks. There is mounting evidence that many explanation methods are rather unreliable and susceptible to malicious manipulations. In this paper, we particularly aim to understand the robustness of explanation methods in the context of text modality. We provide initial insights and results towards devising a successful adversarial attack against text explanations. To our knowledge, this is the first attempt to evaluate the adversarial robustness of an explanation method. Our experiments show the explanation method can be largely disturbed for up to 86% of the tested samples with small changes in the input sentence and its semantics.

==> section3/baselines.tex <==
% Hessel: moved into methods for debugging some issue...


==> section3/definition.tex <==
% Our fundamental hypothesis is that a small change to the input should translate to a minimal change in the explanation. We formalize this as follows. 

In this section, we formally introduce the procedure.
For an input $X$ consisting of a sequence of words $x_1, x_2,\ldots,x_n$ and a model $M$ that produces a prediction $P$, the explanation $E$ is defined as the vector of attributions $e_1, e_2,...,e_n$ produced by applying an explanation method $S$ to $X$ and $M$ where $e_i$ indicates the importance of the word to $M$ in producing $P$. A positive value of $e_i$ indicates that $x_i$ supported the prediction while a negative value indicates that $x_i$ contradicted the prediction.

% We then apply 

We measure the attribution shift using two methods: cosine similarity or $L^\infty$ distance of the .

An explanation method $S$ is \textit{robust} to an attack $A$ on model $M$ if, for most of the inputs $X_i$, the explanation $E_{io}$ generated for the original sample $X_{io}$ is similar to the explanation $E_{ip}$ generated for the perturbed sample $X_{ip}$ which is created by applying $A$ to $X_{io}$.

% In the current experiments, we measure this similarity using the cosine similarity function. Therefore a high cosine similarity for most of the samples indicates that $S$ is robust while a low cosine similarity for most of the samples indicates that $S$ is not robust.

==> section3/explanation_methods.tex <==
An explanation method is a function that receives a model and a model input and maps them to an attribution object of the same size as the input. Each entry in the output of the explanation method describes the relevance of the corresponding entry in the input for predicting the class.
\par We now briefly describe a selection of relevant explanation methods.
\vspace{0.1em} %\todo{Should we keep all of these methods when we're only applying one?}
\\
\textbf{Gradient} method is the simplest among the explanation methods. The gradient of the output is calculated with respect to the input and each gradient serves as the importance of the corresponding feature in input.
\vspace{0.4em}
\\
\textbf{Gradient}~$\bigodot$~\textbf{Input} is an extension of the gradient method. It takes gradients of the output with respect to input and multiplies them by the input feature values. An intuition for this method can be obtained by taking a linear model. The gradients are simply the coefficients of each input, and the product of the input with a coefficient corresponds to the total contribution of the feature to the linear model's output.
\vspace{0.4em}
\\
\textbf{Integrated Gradients (IG)} ~\cite{sundararajan2017axiomatic} addresses gradient saturation by summing over scaled versions of the input. IG for an input x is defined as \\$E_{IG}(x) = (x-\overline{x}) \times \int\limits_0^1\frac{\partial S(\overline{x}+\alpha(x-\overline{x}))}{\partial x}d\alpha$
\\where $\overline{x}$ is a baseline input.
\vspace{0.4em}
\\
\textbf{SmoothGrad (SG)}  ~\cite{smoothgrad} seeks to alleviate noise diffusion for saliency maps by averaging over explanations of noisy copies of an input. This can be used on top of any of the attribution methods.

